Formal Analysis of Galois Field Arithmetics - Parallel Verification and Reverse Engineering

Galois field (GF) arithmetic circuits find numerous applications in communications, signal processing, and security engineering. Formal verification techniques of GF circuits are scarce and limited to circuits with known bit positions of the primary inputs and outputs. They also require knowledge of the irreducible polynomial $P(x)$, which affects final hardware implementation. This paper presents a computer algebra technique that performs verification and reverse engineering of GF($2^m$) multipliers directly from the gate-level implementation. The approach is based on extracting a unique irreducible polynomial in a parallel fashion and proceeds in three steps: 1) determine the bit position of the output bits; 2) determine the bit position of the input bits; and 3) extract the irreducible polynomial used in the design. We demonstrate that this method is able to reverse engineer GF($2^m$) multipliers in \textit{m} threads. Experiments performed on synthesized \textit{Mastrovito} and \textit{Montgomery} multipliers with different $P(x)$, including NIST-recommended polynomials, demonstrate high efficiency of the proposed method.

==> mas_mult_results_RE.tex <==
\begin{table}[!htb]
\scriptsize
\centering
\begin{tabular}{|r|r|r|r|r|}
\hline
\multirow{2}{*}{$m$} & \multicolumn{1}{c|}{\multirow{2}{*}{Irreducible polynomial P(x)}} & \multirow{2}{*}{\# eqns} & \multicolumn{2}{l|}{$RE$ in 16 threads} \\ \cline{4-5} 
 & \multicolumn{1}{c|}{} &  & Runtime(s) & Mem \\ \hline
64 & $x^{64}$+$x^{21}$+$x^{19}$+$x^4$+1 & 21,814 & 9 & 37 MB \\ \hline
96 & $x^{96}$+$x^{44}$+$x^{7}$+$x^2$+1 & 51,412 &  13 & 86 MB \\ \hline
163 & $x^{163}$+$x^{80}$+$x^{47}$+$x^9$+1 & 153,245 & 160 & 253 MB \\ \hline
233 & $x^{233}$+$x^{74}$+1 & 167,803 & 247 & 1.5 GB \\ \hline
283 & $x^{283}$+$x^{12}$+$x^{7}$+$x^5$+1 & 399,688 & 706 & 4.5 GB \\ \hline
409 & $x^{409}$+$x^{87}$+1 & 508,507 & 1327 & 8.3 GB \\ \hline
571 & $x^{571}$+$x^{10}$+$x^{5}$+$x^2$+1 & 1628,170 & 4094 & 27.1 GB \\ \hline
\end{tabular}
\caption{\small Results of reverse engineering Mastrovito multipliers using NIST-recommended polynomials.}
\label{tbl:mas}
\end{table}

==> mont_mult_results_RE.tex <==
\begin{table}[!htb]
\scriptsize
\centering
\begin{tabular}{|r|r|r|r|r|}
\hline
\multirow{2}{*}{$m$} & \multicolumn{1}{c|}{\multirow{2}{*}{Irreducible polynomial P(x)}} & \multirow{2}{*}{\# eqns} & \multicolumn{2}{l|}{$RE$ in 16 threads} \\ \cline{4-5} 
 & \multicolumn{1}{c|}{} &  & Runtime(s) & Mem \\ \hline
64 & $x^{64}$+$x^{21}$+$x^{19}$+$x^4$+1 & 16.898 & 42 & 30 MB\\ \hline
96 & $x^{96}$+$x^{44}$+$x^{7}$+$x^2$+1 & 37,634 & 230 & 119 MB \\ \hline
163 & $x^{163}$+$x^{80}$+$x^{47}$+$x^9$+1 & 107,582 & 1617 & 2.6 GB \\ \hline
233 & $x^{233}$+$x^{74}$+1 & 219,022 & 462 & 4.8 GB \\ \hline
283 & $x^{283}$+$x^{12}$+$x^{7}$+$x^5$+1 & 322,622 & 21525 & 7.8 GB \\ \hline
409 & $x^{409}$+$x^{87}$+1 & 672,396 & - & $MO$ \\ \hline
\end{tabular}
\caption{\small Results of reverse engineering Montgomery multipliers using NIST-recommended polynomials. MO=Out of 32 GB}
\label{tbl:mont}
\end{table}

==> other_px_RE.tex <==
\begin{table}[!htb]
\scriptsize
\centering
\begin{tabular}{|r|r|r|r|}
\hline
\multicolumn{2}{|c|}{Optimal P(x) in GF($2^{233}$)} & Runtime(s) & Mem \\ \hline
\textit{Intel-Pentium} & $x^{233}$+$x^{201}$+$x^{105}$+$x^9$+1 & 549 & 11.7 GB \\ \hline
\textit{ARM} & $x^{233}$+$x^{159}$+1 & 235 & 5.1 GB \\ \hline
\textit{MSP430} & $x^{233}$+$x^{185}$+$x^{121}$+$x^{105}$+1 & 513 & 10.9 GB \\ \hline
\textit{NIST-recommended} & $x^{233}$+$x^{74}$+1 & 263 & 4.8 GB \\ \hline
\end{tabular}
\caption{\small Result of reverse engineering GF($2^{233}$) Mastrovito multipliers that are implemented using different $P(x)$.}
\vspace{-3mm}
\label{tbl:diff_p}
\end{table}
